Improving Crowdsourced Live Streaming with Aggregated Edge Networks

Recent years have witnessed a dramatic increase of user-generated video services. In such user-generated video services, crowdsourced live streaming (e.g., Periscope, Twitch) has significantly challenged today's edge network infrastructure: today's edge networks (e.g., 4G, Wi-Fi) have limited uplink capacity support, making high-bitrate live streaming over such links fundamentally impossible. In this paper, we propose to let broadcasters (i.e., users who generate the video) upload crowdsourced video streams using aggregated network resources from multiple edge networks. There are several challenges in the proposal: First, how to design a framework that aggregates bandwidth from multiple edge networks? Second, how to make this framework transparent to today's crowdsourced live streaming services? Third, how to maximize the streaming quality for the whole system? We design a multi-objective and deployable bandwidth aggregation system BASS to address these challenges: (1) We propose an aggregation framework transparent to today's crowdsourced live streaming services, using an edge proxy box and aggregation cloud paradigm; (2) We dynamically allocate geo-distributed cloud aggregation servers to enable MPTCP (i.e., multi-path TCP), according to location and network characteristics of both broadcasters and the original streaming servers; (3) We maximize the overall performance gain for the whole system, by matching streams with the best aggregation paths.

==> Makefile <==
doc=main

all: $(doc).pdf

$(doc).pdf: *.tex sections/*.tex figures/*
	xelatex $(doc)

compile:
	xelatex $(doc)
	bibtex $(doc)
	xelatex $(doc)
	xelatex $(doc)

clean:
	rm -rf $(DOCUMENT).ps *.aux *.toc *.pdf \
	*.blg *.bbl *.blg *.dvi *.mtc *.mtc? *.maf *.log *.out


==> sections/relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}


Bandwidth efficiency, quality stability and resource fairness are the primary goals users want to achieve in a multimedia streaming system.

\subsection{Crowdsourced Video Sharing}

\subsection{Bandwidth Aggregation}

What is the gap

